Differentially-Private Heat and Electricity Markets Coordination

Sector coordination between heat and electricity systems has been identified has an energy-efficient and cost-effective way to transition towards a more sustainable energy system. However, the coordination of sequential markets relies on the exchange of sensitive information between the market operators, namely time series of consumers' loads. To address the privacy concerns arising from this exchange, this paper introduces a novel privacy-preserving Stackelberg mechanism (w-PPSM) which generates differentially-private data streams with high fidelity. The proposed w-PPSM enforces the feasibility and fidelity of the privacy-preserving data with respect to the original problem through a post-processing phase in order to achieve a close-to-optimal coordination between the markets. Multiple numerical simulations in a realistic energy system demonstrate the effectiveness of the w-PPSM, which achieves up to two orders of magnitude reduction in the cost of privacy compared to a traditional differentially-private mechanism.

==> custom_commands.tex <==
%!TEX root=main.tex
% Use the postscript times font!
\usepackage{times}
\renewcommand*\ttdefault{txtt}
\usepackage{soul}
\usepackage{url}
\usepackage[hidelinks]{hyperref}
\usepackage[utf8]{inputenc}
\usepackage[small]{caption}
\usepackage{subcaption}
\urlstyle{same}

\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{booktabs}
\usepackage{graphicx}

% insert here the call for the packages your document requires
\usepackage[ruled,linesnumbered,noresetcount,vlined]{algorithm2e}
\renewcommand\AlCapNameSty{\slshape}
\SetKwFor{Repeat}{repeat}{:}{endw}
\usepackage{amsmath,amsfonts,mathrsfs,amssymb,bm,mathtools,mathabx}
\usepackage{graphicx, epsfig, epstopdf}
\usepackage{wrapfig, multirow, multicol,mdframed}
\usepackage{rotating, booktabs}
\usepackage{stmaryrd,xspace,arydshln}
\usepackage{picinpar}
\usepackage{todonotes}
\usepackage{color}
\usepackage{enumitem}
\usepackage{cleveref}

\usepackage{float}
\floatstyle{ruled}
\newfloat{model}{thp}{lop}
\floatname{model}{Model}
\newcounter{models}
\newcommand{\cc}[2]{\multicolumn{1}{#1}{#2}}
\newcommand{\citep}[1]{\citeauthor{#1}~[\citeyear{#1}]}

